Maximizing Nash Social Welfare in 2-Value Instances

We consider the problem of maximizing the Nash social welfare when allocating a set $\mathcal{G}$ of indivisible goods to a set $\mathcal{N}$ of agents. We study instances, in which all agents have 2-value additive valuations: The value of every agent $i \in \mathcal{N}$ for every good $j \in \mathcal{G}$ is $v_{ij} \in \{p,q\}$, for $p,q \in \mathbb{N}$, $p \le q$. Maybe surprisingly, we design an algorithm to compute an optimal allocation in polynomial time if $p$ divides $q$, i.e., when $p=1$ and $q \in \mathbb{N}$ after appropriate scaling. The problem is \classNP-hard whenever $p$ and $q$ are coprime and $p \ge 3$. In terms of approximation, we present positive and negative results for general $p$ and $q$. We show that our algorithm obtains an approximation ratio of at most 1.0345. Moreover, we prove that the problem is \classAPX-hard, with a lower bound of $1.000015$ achieved at $p/q = 4/5$.

==> missing-proofs.tex <==
\section{Missing Proofs}
\subsection{Missing Proofs of Section \ref{prelim}}
\reachableAgentMoreBigGoods*
\begin{proof}
	Assume for contradiction that it is not true. Then for every agent $j$ that is reachable from $i$ by a {\sf BB}-balancing path it holds that $b_j \leq  b^*_j$. We denote by $C$ the set of these reachable agents, $i$ included. Let $\delta_j^{-}$ and $\delta_j^{+}$ be the in/out-degree of $j$, respectively, in the subgraph of $\transGraph{O^*}{O}$ induced by $C$. Observe that $\delta_j^{+}$ is at least the number of big goods given away by $j$ when comparing $O^*$ to $O$. Similarly, $\delta_j^{-}$ is at most the number of big goods agent $j$ receives in this comparison. Thus, $b^*_j \leq b_j + \delta_j^{+} -\delta_j^{-}$ for each $j\in C$. By assumption $b_j \leq b^*_j$ for each $j\in C\setminus \set{i}$, we see $\delta_j^{+} -\delta_j^{-} \geq 0$. Since $\sum_{j\in C} \delta_j^{+} = \sum_{j\in C} \delta_j^{-} $, we have $b^*_i - b_i \leq \delta_i^{+} - \delta_i^{-} \leq 0$ -- a contradiction to $b_i  < b^*_i$. Hence, a reachable agent $j \in C$ with $b_j^* < b_j$ must exist.
\end{proof}

\reachableAgentLessBigGoods*
\begin{proof}
We denote by $C$ the set of agents that can reach $j$ through a balancing path, $j$ included. Let $\delta_i^{-}$ and $\delta_i^{+}$ be the in/out-degree of agent $i$ in the subgraph induced by $C$. We show that if in the induced subgraph there is no \SB-balancing path ending in $j$, then there must exist agent $i \in C$ such that $b_i^* > b_i$. Then, since $i \in C$ and $\transGraph{O^*}{O}$ neither has \SS- nor \BS-balancing paths, there must be a \BB-balancing path in $\transGraph{O^*}{O}$.

First, suppose there is at least one ``\SB-edge'' among agents in $C$, i.e., a pair $(\ell,\ell') \in E_{O^* \to O}$ with $\ell, \ell' \in C$, $g(\ell,\ell') \in S_{\ell}$, and $g(\ell,\ell') \in B_{\ell'}$. Clearly, by construction there is an \SB- or \BB-balancing path from $\ell'$ to $j$. If it is a \BB-balancing path, by extending it with edge $(\ell,\ell')$ we obtain an \SB-balancing path from $\ell$ to $j$. Hence, property (1) of the lemma holds.

Now suppose there is no ``\SB-edge'' among agents in $C$. Then there can be no \SB-balancing path in the subgraph induced by $C$. For each $i\in C$, $\delta_i^{+}$ is at most the number of big goods given away by $i$ when comparing $O^*$ to $O$. Now in $O$ no small good is assigned. Hence, by the construction of $C$, we see $\delta_i^{-}$ exactly corresponds to the number of big goods agent $i$ receives when changing $O^*$ to $O$, for each $i\in C$. Similar to the proof of \Cref{lemma:reachableAgentMoreBigGoods}, the connection between degrees and the vectors $b$ and $b^*$ implies property (2) of the lemma.
\end{proof}

\subsection{Missing Proofs of Section \ref{optimal}}

\propertiesAlgo*
\begin{proof}
	We show the properties inductively. For the base case, we observe that they hold before the beginning of phase 3 (i.e., in a round 0 of phase 3). Since we allocated small goods greedily in phase 2, all agents $i,j$ with small goods in their bundle satisfy $v_i(A_i) \le \min_{j \in \agents} v_j(A_j) + v$. The properties (1)-(3) hold trivially before the beginning of phase 3, since the condition is not fulfilled and there are no earlier rounds. In other words, Properties (1)-(3) are empty for $t = 0$.
	%
	%Hence, if $i_1^1$ has a small good, moving any good is not profitable for the NSW, so $i_1^1$ must have only big goods (1). Clearly, in the first round of phase 3 we have (2).} Suppose $g \in A_{i_1^1}$ is big for $i_2^1$ and a move strictly improves the NSW. Then, since the valuation of $i_2^1$ only increased during phase 2, it must have been possible to improve $O$, either in terms of the number of agents receiving big goods, or in terms of NSW of agents with non-empty bundle. This is a contradiction and proves (3).
	
	Now assume that all properties hold until round $t-1 \ge 0$ of phase 3 and consider round $t$. Clearly, when the hypothesis holds, the valuation of agents that have only big goods is decreasing, while the valuation of agents with small goods is increasing. Moreover, since the target agent has minimum valuation and receives a small good, all agents with small goods have valuation at most $\min_{j \in \agents} v_j(A_j) + v$. As a consequence, if $i_1^t$ in round $t$ has a small good, then moving any good is not profitable for the NSW, so we have (1). Suppose we moved a good from $i_2^t$ in an earlier round $t'$, i.e., $i_2^t = i_1^{t'}$. By hypothesis for round $t'$, $i_1^{t'}$ was the agent with highest valuation and had only big goods in round $t'$; moreover, for rounds $t'+1,\ldots,t-1$, the valuation of $i_1^t$ and $i_2^t = i_1^{t'}$ at the beginning of round $t$ can differ by at most 1. Then a move of a good from $i_1^t$ to $i_2^t$ is not profitable, which proves (2). Finally, suppose $g \in A_{i_1^t}$ is big for $i_2^t$. Then, since $i_2^t$ never lost a good up to round $t$, the valuation of $i_2^t$ only increased since the end of phase 1. As such, it must have been possible to improve $O$, either in terms of the number of agents receiving big goods, or in terms of NSW of agents with non-empty bundles. This is a contradiction and shows (3).
%	\textcolor{blue}{If at the end of round $t$ we have an agent $i$ with a small good and $v_i(A_i) > \min_{j \in \agents} v_j(A_j)+v$, then as $i_2^t$ received a good, we have $v_{i_2^t}(A^{i_2^t}_{i_2^t}) > \min_{j \in \agents} v_j(A_j)+v$. But the only agent whose valuation decreased is $i^t_1$, so $\min_{j \in \agents} v_j(A_j) = v_{i_1^t}(A^{i_1^t}_{i_1^t})$. Thus, before round $t$, the valuations of $i_1^t$ and $i_2^t$ differed by less than $1$, so moving the good did not increase the NSW, a contradiction.}
\end{proof}


\Cref{lemma:reachableAgentMoreBigGoods} can be combined with \Cref{prop:bigGoodsInOpt} to yield the following corollary.

\begin{corollary}
	\label{cor:bigGoodsInOpt}
	If there is an agent $i$ with $b_i < b_i^*$, then there is some agent $j$ reachable from $i$ by a \BB-balancing path in $\transGraph{O^*}{O}$. Every such agent $j$ has at least one small good in $O^*_j$.
\end{corollary}
